CORAL8: Concurrent Object Regression for Area Localization in Medical Image Panels

This work tackles the problem of generating a medical report for multi-image panels. We apply our solution to the Renal Direct Immunofluorescence (RDIF) assay which requires a pathologist to generate a report based on observations across the eight different WSI in concert with existing clinical features. To this end, we propose a novel attention-based multi-modal generative recurrent neural network (RNN) architecture capable of dynamically sampling image data concurrently across the RDIF panel. The proposed methodology incorporates text from the clinical notes of the requesting physician to regulate the output of the network to align with the overall clinical context. In addition, we found the importance of regularizing the attention weights for word generation processes. This is because the system can ignore the attention mechanism by assigning equal weights for all members. Thus, we propose two regularizations which force the system to utilize the attention mechanism. Experiments on our novel collection of RDIF WSIs provided by a large clinical laboratory demonstrate that our framework offers significant improvements over existing methods.

==> conclusions.tex <==
\section{Conclusions}
\label{section:Conclusions}
The performance of generative models can be greatly improved by conditioning the model on clinical note features and regulating alpha attention weights to pay equal attention to each image in the set.

==> related_works.tex <==
\section{Related Works}
\label{section:relatedworks}
This section provides relevant background to the \emph{image captioning with attention} methods explored in this paper. Specifically we address previous works related to attention regularisation and automatically generating medical image reports.\\
\\
\textbf{Automated medical reporting} Yuan Xue et al~\cite{compare} describe an architecture capable of taking the frontal and lateral views of a radiology image as input to generate a multi-sentence paragraph description. They implement a sentence level recurrent attention mechanism to produce a conditioning image context vector for their LSTM network. This method appears to have achieved admirable quantitative performance, but their are several limitations which make it ineffective for the RDIF medical report generation task. As this is a multi-view task, both images are assumed to represent the same object. Hence, there are no constraints to preserve the individualism of images in the pair: discriminatory features can be extracted from either image to represent the set. This assumption is inappropriate for the RDIF dataset as each image contains a unique interpretable object:  the state of images in the set cannot be extrapolated from discriminatory features identified in a single image. Their have been many proposed solutions to the problem of automatically reporting medical tests~\cite{mdnet, tienet, compare} but to our knowledge, none of these methods exploit clinical observations available at the time of testing. As such, there are currently no methods equipped to handle the clinical context bias described in section~\ref{section:introduction}.\\
\\
\textbf{Attention Regularization} Xu et al~\cite{xu} implement a doubly stochastic regularization strategy to supervise the outputs of the attention network. This encourages network to pay equal attention to all regions of an image over the generative sequence. However, their are no constraints in place to prevent invariant uniformly distributed patterns of attention. As such, the attention network may be able to effectively discriminate samples in training data without identifying the generalizable features representative of their class.\\
\\
